Towards Multiphase Clocking in Single-Flux Quantum Systems

Rapid single-flux quantum (RSFQ) is one of the most advanced superconductive electronics technologies. SFQ systems operate at tens of gigahertz with up to three orders of magnitude smaller power as compared to CMOS. In conventional SFQ systems, most gates require clock signal. Each gate should have the fanins with equal logic depth, necessitating insertion of path-balancing (PB) DFFs, incurring prohibitive area penalty. Multiphase clocking is the effective method for reducing the path-balancing overhead at the cost of reduced throughput. However, existing tools are not directly applicable for technology mapping of multiphase systems. To overcome this limitation, in this work, we propose a technology mapping tool for multiphase systems. Our contribution is threefold. First, we formulate a phase assignment as a Constraint Programming with Satisfiability (CP-SAT) problem, to determine the phase of each element within the network. Second, we formulate the path balancing problem as a CP-SAT to optimize the number of DFFs within an asynchronous datapath. Finally, we integrate these methods into a technology mapping flow to convert a logic network into a multiphase SFQ circuit. In our case studies, by using seven phases, the size of the circuit (expressed as the number of Josephson junctions) is reduced, on average, by 59.94 % as compared to the dual (fast-slow) clocking method, while outperforming the state-of-the-art single-phase SFQ mapping tools.

==> table_dcm.tex <==
\begin{table}[h]
\setlength\tabcolsep{2pt}
\centering
\caption{Comparison of multiphase clocking with dual clocking method \cite{dual_clock} with 20\% throughput}
\begin{tabular}{r|rrr|rrr|r}
\toprule 
          & \multicolumn{3}{c|}{Multiphase (our work)}                                      & \multicolumn{3}{c|}{Dual clocking method \cite{dual_clock}}  &              \\
\cmidrule(rl){1-1} \cmidrule(rl){2-4} \cmidrule(rl){5-7} \cmidrule(rl){8-8}
          & \multicolumn{1}{r|}{DFF}   & \multicolumn{1}{r|}{JJ}     & \hsc{Latency} & \multicolumn{1}{r|}{DFF}   & \multicolumn{1}{r|}{NDRO} & \hsc{Latency} & Impr. \% \\
\cmidrule(rl){1-1} \cmidrule(rl){2-4} \cmidrule(rl){5-7} \cmidrule(rl){8-8}
\cf{sin}       & \multicolumn{1}{r|}{11,170} & \multicolumn{1}{r|}{121,350} & 17      & \multicolumn{1}{r|}{13,581} & \multicolumn{1}{r|}{24}   & 186   & 17.8      \\
\rowcolor{gray!15}
\cf{int2float} & \multicolumn{1}{r|}{258}   & \multicolumn{1}{r|}{4,239}   & 2       & \multicolumn{1}{r|}{139}   & \multicolumn{1}{r|}{11}   & 16    & -85.6     \\
\cf{priority}  & \multicolumn{1}{r|}{7,567}  & \multicolumn{1}{r|}{62,490}  & 17      & \multicolumn{1}{r|}{21,115} & \multicolumn{1}{r|}{128}  & 249   & 64.2      \\
\rowcolor{gray!15}
\cf{i2c}       & \multicolumn{1}{r|}{1,208}  & \multicolumn{1}{r|}{21,663}  & 3       & \multicolumn{1}{r|}{1,544}  & \multicolumn{1}{r|}{147}  & 17    & 21.8      \\
\cf{voter}     & \multicolumn{1}{r|}{4,353}  & \multicolumn{1}{r|}{147,638} & 8       & \multicolumn{1}{r|}{6,716}  & \multicolumn{1}{r|}{1,001} & 71    & 35.2      \\
\rowcolor{gray!15}
\cf{c432}      & \multicolumn{1}{r|}{443}   & \multicolumn{1}{r|}{4,555}   & 4       & \multicolumn{1}{r|}{447}   & \multicolumn{1}{r|}{36}   & 24    & 0.9       \\
\cf{c499}      & \multicolumn{1}{r|}{242}   & \multicolumn{1}{r|}{4,691}   & 2       & \multicolumn{1}{r|}{218}   & \multicolumn{1}{r|}{41}   & 13    & -11.0     \\
\rowcolor{gray!15}
\cf{c1908}     & \multicolumn{1}{r|}{212}   & \multicolumn{1}{r|}{3,593}   & 3       & \multicolumn{1}{r|}{473}   & \multicolumn{1}{r|}{33}   & 20    & 55.2      \\
\cf{c3540}     & \multicolumn{1}{r|}{812}   & \multicolumn{1}{r|}{14,456}  & 4       & \multicolumn{1}{r|}{795}   & \multicolumn{1}{r|}{50}   & 32    & -2.1      \\
\rowcolor{gray!15}
\cf{c5315}     & \multicolumn{1}{r|}{1,050}  & \multicolumn{1}{r|}{22,735}  & 3       & \multicolumn{1}{r|}{2,554}  & \multicolumn{1}{r|}{178}  & 27    & 58.9      \\
\cf{c7552}     & \multicolumn{1}{r|}{847}   & \multicolumn{1}{r|}{17,722}  & 4       & \multicolumn{1}{r|}{1,912}  & \multicolumn{1}{r|}{207}  & 21    & 55.7      \\
\rowcolor{gray!15}
\multicolumn{1}{r}{Average}   & \multicolumn{1}{r}{}      & \multicolumn{1}{r}{}       &    \multicolumn{1}{r}{}     & \multicolumn{1}{r}{}      & \multicolumn{1}{r}{}     &      & 19.2      \\
\bottomrule
\end{tabular}\label{tab:with_dcm}
\end{table}

% \hsc{benchmark} & \hsc{\#DFF} & \hsc{\#JJ}    & \hsc{Depth} & \hsc{\#DFF} & \hsc{Impr.} & \hsc{\#JJ} & \hsc{Impr.} & \hsc{Depth} & \hsc{Impr.} & \hsc{Runtime, s} \\

==> table_dcm_2.tex <==
\begin{table*}[h]
\setlength\tabcolsep{4pt}
\centering
\caption{Comparison of multiphase clocking with dual clocking method \cite{dual_clock} for different throughputs}
\vspace{-1em}
\begin{tabular}{l|rrrrrr|rrrrrr}
               & \mcl{6}{c|}{1/7 throughput}                                                              & \mcl{6}{c}{1/12 throughput}                                                                 \\
\cmidrule(rl){2-7} \cmidrule(rl){8-13}
               & \mcl{2}{c}{DCM}                 & \mcl{2}{c}{Multiphase}           & \mcl{2}{c|}{Change}  & \mcl{2}{c}{DCM}                    & \mcl{2}{c}{Multiphase}          & \mcl{2}{c}{Change}    \\
               & \#DFF  & \#JJ                   & \#DFF   & \#JJ                   & \#DFF    & \#JJ     & \#DFF     & \#JJ                   & \#DFF  & \#JJ                   & \#DFF     & \#JJ     \\
\cmidrule(rl){2-3} \cmidrule(rl){4-5} \cmidrule(rl){6-7} \cmidrule(rl){8-9} \cmidrule(rl){10-11} \cmidrule(rl){12-13}
\cf{int2float} & 117    & \mcl{1}{r|}{7'770}     & 217     & \mcl{1}{r|}{5'136}     & +85.47\% &--33.90\% & 39        & \mcl{1}{r|}{5'140}     & 46     & \mcl{1}{r|}{3'939}     & +17.95\%  &--23.37\% \\
\rowcolor{gray!15}
\cf{priority}  & 8'562  & \mcl{1}{r|}{257'252}   & 3'285   & \mcl{1}{r|}{45'094}    &--61.63\% &--82.47\% & 4'225     & \mcl{1}{r|}{158'568}   & 1'775  & \mcl{1}{r|}{34'524}    &--57.99\%  &--78.23\% \\
\cf{voter}     & 7'204  & \mcl{1}{r|}{447'044}   & 2'180   & \mcl{1}{r|}{162'804}   &--69.74\% &--63.58\% & 3'732     & \mcl{1}{r|}{355'144}   & 1'568  & \mcl{1}{r|}{158'520}   &--57.98\%  &--55.36\% \\
\rowcolor{gray!15}
\cf{c432}      & 224    & \mcl{1}{r|}{10'734}    & 342     & \mcl{1}{r|}{5'116}     & +52.68\% &--52.34\% & 118       & \mcl{1}{r|}{7'124}     & 240    & \mcl{1}{r|}{4'402}     & +103.39\% &--38.21\% \\
\cf{c880}      & 362    & \mcl{1}{r|}{14'658}    & 254     & \mcl{1}{r|}{6'190}     &--29.83\% &--57.77\% & 187       & \mcl{1}{r|}{9'483}     & 119    & \mcl{1}{r|}{5'245}     &--36.36\%  &--44.69\% \\
\rowcolor{gray!15}
\cf{c1908}     & 282    & \mcl{1}{r|}{13'169}    & 125     & \mcl{1}{r|}{3'529}     &--55.67\% &--73.20\% & 144       & \mcl{1}{r|}{8'739}     & 69     & \mcl{1}{r|}{3'137}     &--52.08\%  &--64.10\% \\
\cf{c3540}     & 776    & \mcl{1}{r|}{43'437}    & 589     & \mcl{1}{r|}{17'016}    &--24.10\% &--60.83\% & 282       & \mcl{1}{r|}{26'897}    & 440    & \mcl{1}{r|}{15'973}    & +56.03\%  &--40.61\% \\
\rowcolor{gray!15}
\cf{c1355}     & 193    & \mcl{1}{r|}{8'739}     & 46      & \mcl{1}{r|}{4'515}     &--76.17\% &--48.34\% & 119       & \mcl{1}{r|}{6'149}     & 44     & \mcl{1}{r|}{4'501}     &--63.03\%  &--26.80\% \\
\cf{s13207}    & 1'795  & \mcl{1}{r|}{106'346}   & 1'837   & \mcl{1}{r|}{42'382}    & +2.34\%  &--60.15\% & 571       & \mcl{1}{r|}{60'766}    & 1'082  & \mcl{1}{r|}{37'097}    & +89.49\%  &--38.95\% \\
\rowcolor{gray!15}
\cf{s5378}     & 645    & \mcl{1}{r|}{50'766}    & 808     & \mcl{1}{r|}{21'761}    & +25.27\% &--57.13\% & 255       & \mcl{1}{r|}{34'053}    & 368    & \mcl{1}{r|}{18'681}    & +44.31\%  &--45.14\% \\
\cf{s382}      & 56     & \mcl{1}{r|}{4'448}     & 89      & \mcl{1}{r|}{2'411}     & +58.93\% &--45.80\% & 9         & \mcl{1}{r|}{2'750}     & 48     & \mcl{1}{r|}{2'124}     & +433.33\% &--22.76\% \\
\cmidrule(rl){1-1} \cmidrule(rl){2-7} \cmidrule(rl){8-13}
Geomean        & 557.04 & \mcl{1}{r|}{29'868.20} & 413.48  & \mcl{1}{r|}{11'965.54} &--25.77\% &--59.94\% & 227.85    & \mcl{1}{r|}{19'565.38} & 229.57 & \mcl{1}{r|}{10'467.10} & +0.76\%   &--46.50\% 
\end{tabular}\label{tab:with_dcm}
\end{table*}
